AIOpsLab: A Holistic Framework to Evaluate AI Agents for Enabling Autonomous Clouds

AI for IT Operations (AIOps) aims to automate complex operational tasks, such as fault localization and root cause analysis, to reduce human workload and minimize customer impact. While traditional DevOps tools and AIOps algorithms often focus on addressing isolated operational tasks, recent advances in Large Language Models (LLMs) and AI agents are revolutionizing AIOps by enabling end-to-end and multitask automation. This paper envisions a future where AI agents autonomously manage operational tasks throughout the entire incident lifecycle, leading to self-healing cloud systems, a paradigm we term AgentOps. Realizing this vision requires a comprehensive framework to guide the design, development, and evaluation of these agents. To this end, we present AIOPSLAB, a framework that not only deploys microservice cloud environments, injects faults, generates workloads, and exports telemetry data but also orchestrates these components and provides interfaces for interacting with and evaluating agents. We discuss the key requirements for such a holistic framework and demonstrate how AIOPSLAB can facilitate the evaluation of next-generation AIOps agents. Through evaluations of state-of-the-art LLM agents within the benchmark created by AIOPSLAB, we provide insights into their capabilities and limitations in handling complex operational tasks in cloud environments.

==> 0abstract.tex <==
AI for IT Operations (AIOps) aims to automate complex operational tasks, such as fault localization and root cause analysis, to reduce human workload and minimize customer impact. Traditionally, DevOps tools and AIOps algorithms focus on different isolated operational tasks. However, the rapid recent advancements in Large Language Models (LLMs) and AI agents are revolutionizing AIOps by enabling end-to-end and multitask automation. In this paper, we envision a future where AI agents can seamlessly handle different types of operational tasks across the incident lifecycle stack and achieve an autonomous, self-healing cloud systems, creating a new paradigm termed Agent for Operations, i.e., AgentOps. To realize this vision, a holistic framework is needed to empower evaluating these agents. We contribute to this goal by proposing and implementing an evaluation framework, AIOpsLab, that allows users to design, build, and assess the effectiveness and efficiency of agents in cloud environments, e.g., microservices. This paper discusses the essential requirements for such a holistic framework and proposes AIOpsLab, which orchestrates applications, injects fine-grained, realistic faults to the cloud, and interfaces with agents. By evaluating state-of-the-art AIOps LLM agents within AIOpsLab, we provide an analysis that offers valuable insights into their capabilities and limitations in handling complex operational tasks in cloud environments.





==> 2aci.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{Figures/bg.pdf}
    \caption{Microservice incident and its management lifecycle.} %
    \label{fig:intro}
  \end{figure}

In this section, we discuss the design principles 
    that a holistic, standardized framework needs
    to evaluate AIOps agents.
A key objective is to create an effective \textbf{Agent Cloud Interface (ACI)}, 
    which facilitates interaction between agents and cloud systems. 
Inspired by human/agent-computer interaction principles~\cite{swebench,sweagent}, 
    the ACI should simplify cloud operations, 
    allowing agents to communicate, take action, 
    and receive feedback from cloud services efficiently. 
The ACI acts as an orchestrator, 
    managing these interactions 
    and enabling agents to detect and resolve issues 
    in dynamic cloud environments.
We build on existing principles~\cite{shetty2024buildingaiagentsautonomous},
    and list the key design decisions 
    shaping the ACI's structure and functionality here.

\textit{Unified Interaction with Cloud Services.}
The ACI provides a consistent, standardized interface 
    for interacting with cloud services, 
    whether it's used by different agents or even human operators.
The ACI is designed to present a consistent, 
    unified interface for interacting with cloud services. 
Through clearly defined APIs, the ACI exposes key actions 
    to agents,
    like retrieving logs, gathering metrics, 
    and executing commands.

\textit{Real-time, Actionable Feedback.}  
Another design aspect of the ACI is its ability 
    to provide meaningful and actionable feedback 
    for every action taken by the agent. 
After each action, whether successful or not, 
    the system generates detailed feedback, 
    including error messages, system responses, and output logs,
    so that agents can adjust their next action on the fly. 

\textit{Simplified Action Space.} 
The cloud is a complex environment 
    with numerous services and operations.
Without a clear list of actions, 
    agents may struggle to navigate the cloud.
The ACI should simplify the action space into a clear 
    and manageable list of valid API calls, 
    e.g., Kubernetes or telemetry scraping commands.


    










==> 2background.tex <==




\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{Figures/bg.pdf}
  \caption{Cloud Incident Management Lifecycle.} %
  \label{fig:intro}
\end{figure}




















Current benchmarks suffer from several key limitations, 
  making it challenging to effectively evaluate LLM-based AIOps agents.
Existing benchmarks are mostly static, 
  providing datasets such as Key Performance Indicators (KPIs) 
  or system metrics~\cite{adbench,anomalybench}, i.e., time series data, 
  or fixed question-answer format~\cite{opseval} 
  that often do not reflect the dynamic nature of real-world cloud environments. 
These static benchmarks can be limited in fidelity, 
  failing to replicate the unpredictable and evolving conditions 
  found in production systems and incident management process. 

Second, there is also a lack of clear task definitions, 
  particularly concerning the types of faults introduced. 
Though there are many fault injection tools for testing the resilience of cloud systems~\cite{marinescu2009lfi,Banabic2012,Christakis2017a,zhang2012amplifying,jepsen, Pillai2014,alquraan2018analysis,lu2019crashtuner, chen2020cofi, leesatapornwongsa2014samc, gunawi2011fate, majumdar2018why, Ju2013, heorhiadi2016gremlin,alagappan2016correlated,Mohan2018,sun:osdi:22,canini2012nice}, 
  many benchmarks focus solely on injecting system symptoms 
  with existing fault injector~\cite{chaosblade,chaosmesh}, 
  such as pod failure, high CPU utilization or network latency. 
These coarse-grained faults in the existing benchmarks 
  can only cause disruption without modeling the underlying, 
  fine-grained root causes~\cite{lu2019crashtuner, chen2020cofi, leesatapornwongsa2014samc,Mohan2018,sun:osdi:22,gu:sosp:23}. 
They cannot evaluate true capabilities of AIOps agents 
  to diagnose and mitigate root causes, 
  limiting people to understand how well these agents perform 
  at different types of the incident tasks.
However, to evaluate AIOps agents effectively, 
  the failure scenarios must go beyond simple performance or crash failures. 
Instead, they should reflect realistic cases that challenge the agents' ability.


























==> 3.2fault.tex <==
\subsection{Problem Pool}
To effectively assess different AIOps approaches, we design evaluation scenarios (which we refer it as \textit{problem}) that replicate realistic incidents. These scenarios involve deliberately introducing faults at various system levels, simulating the diverse operational challenges that AIOps tools and human operators must address.


We present a task level taxonomy that categorizes the tasks that AIOps agent should accomplish according to different stages of the incident management lifecycle, with progressively increasing complexity. Our claim is that the higher level the task is, the harder or more importance of the task can provide to evaluate the agents. This taxonomy provides a structured framework for evaluating how AIOps approaches, be they AI agents, traditional algorithms, or human teams, detect, localize, analyze, and mitigate issues in complex cloud environments. 
\autoref{tab:fault_taxonomy} summarizes the levels of task.


\begin{table}[h]
\centering
\caption{Task taxonomy for AIOps agent evaluation. \textmd{The lower the level, the easier the task. \ourbench{} aims to evaluate agents across all task levels with its problems.}}
\label{tab:fault_taxonomy}
\renewcommand{\arraystretch}{1.2} %
\scriptsize
\vspace{0.25em}
\begin{tabular}{l|l|p{4cm}}
\toprule
\textbf{Level} & \textbf{Task (\# sub tasks)} & \textbf{Evaluation Focus}                                                   \\ \hline
1 & Detection (1) & Can the approach accurately detect anomalies or deviations?                                      \\ \hline
2 & Localization (1) & Can the approach pinpoint the exact source (e.g., microservice) of a fault? \\ \hline
3 & Root Cause Analysis (2) & Can the approach determine the underlying cause of the fault? \\ \hline
4 & Mitigation (1) & Can the approach give effective solutions to recover the environment? \\ \hline
\end{tabular}
\end{table}


Though there are many fault injection tools for testing the resilience of cloud systems~\cite{marinescu2009lfi,Banabic2012,Christakis2017a,zhang2012amplifying,jepsen, Pillai2014,alquraan2018analysis,lu2019crashtuner, chen2020cofi, leesatapornwongsa2014samc, gunawi2011fate, majumdar2018why, Ju2013, heorhiadi2016gremlin,alagappan2016correlated,Mohan2018,sun:osdi:22,canini2012nice}, 
  many benchmarks focus solely on injecting system symptoms 
  with existing fault injector~\cite{chaosblade,chaosmesh}, 
  such as pod failure, high CPU utilization or network latency. 
These coarse-grained faults in the existing benchmarks 
  can only cause disruption without modeling the underlying, 
  fine-grained root causes~\cite{lu2019crashtuner, chen2020cofi, leesatapornwongsa2014samc,Mohan2018,sun:osdi:22,gu:sosp:23}. 
They cannot evaluate true capabilities of AIOps agents 
  to diagnose and mitigate root causes, 
  limiting people to understand how well these agents perform 
  at different types of the incident tasks.
However, to evaluate AIOps agents effectively, 
  the failure scenarios must go beyond simple performance or crash failures. 
Instead, they should reflect realistic cases that challenge the agents' ability.


\textit{Level 1: Detection Ability.}
The foundational requirement for any AIOps approach is the ability to detect anomalies. Level 1 focuses on the preliminary identification of unusual behavior within the system. For example, detecting a sudden spike in CPU usage or an unexpected drop in network throughput indicates deviations from normal operations. Effective detection serves as the first line of defense, enabling the cloud systems to mark the symptoms and flag potential problems.


\textit{Level 2: Localization Ability.}
Once an anomaly is detected, the next step is to localize the fault within the system. Level 2 assesses the ability to accurately determine which component, such as a specific microservice, is malfunctioning. For instance, if a particular service is down, the approach should pinpoint that service rather than attributing the issue to the entire system. Effective localization is crucial for prompt and precise intervention, reducing the time and resources spent on diagnosing issues.


\textit{Level 3: Root Cause Analysis Ability.}
Level 3 evaluates whether the approach can diagnose why a service or component has failed. For example, if a microservice crashes due to an unhandled exception, the method should identify the fault type, i.e., code defect, causing the failure. This level challenges the approach to go beyond surface symptoms and provide insights into the root problem.
\ms{mention the sub problems?}
Note that there could be sub-tasks to form sub-problems.
For example, the root cause analysis task has both the system level
    and fault type sub-problems to be solved.






\textit{Level 4: Resolution and Mitigation.}
The final level assesses the ability to take effective corrective actions. Level 4 evaluates whether the approach can resolve issues by applying appropriate solutions. Key factors include the automation of the resolution process (if applicable) and the specificity and actionability of the proposed solutions. For example, if the root cause is a misconfigured microservice, the approach should adjust its configuration to restore normal operations of that specific microservice instead of re-configure everything. It is crucial to resolve the issue without introducing side effects, such as causing additional faults elsewhere in the system. Additionally, the agent must avoid getting stuck in a loop or taking an excessive amount of time, which could lead to non-termination.










==> 6detection.tex <==
\subsubsection{Detection Task}


In the detection task, the agents were required to identify
    the presence of faults in real-time, 
    without the need to pinpoint the exact fault location.
The task was framed as a binary classification, 
    where the agents had to respond either ``yes'' 
    if a fault was present or ``no'' if it was not.
The results are shown in Table~\ref{tab:metrics_detection}. 


Among the agents, the \gptfourshell{} agent demonstrated 
    the fastest average execution time at 7 seconds.
Although the backend model of \gptthreeshell{}, \gptthreefiveturbo{}, 
    responds faster than \gptfour{}, 
    \gptthreeshell{} needed nearly 10 additional steps on average
    to complete its tasks and had the lowest detection accuracy.
This is attributed to \gptthreeshell{} consistently generating 
    incorrect command formats,
    such as incorrect \texttt{Kubectl} commands, 
    and repeating the same error in subsequent steps.
In many cases, \gptthreeshell{} would repeatedly 
    generate the same incorrect command, 
    often responding with: ``I apologize for the error. Here is the API call again:''
    followed by the same mistake. 
This issue was observed as many as 14 times within a 20-step task.

Similar issues with invalid API formats were also observed in other agents.
For instance, the \react{} agent occasionally generated incorrect API commands
    but typically recovered by reasoning through the errors and self-correcting its commands, 
    as demonstrated in the following example.

\begin{tcolorbox}[
    title={\reactname{} Self-correction Example}, 
    fontupper=\scriptsize,
    fonttitle=\scriptsize,
    sharp corners,               
    boxrule=0.5pt,
    boxsep=1.5pt,
    left=2pt,             
    right=2pt,        
    top=2pt,
    bottom=2pt 
    ]
\reactname{}: \texttt{get\_logs("test-social-network", \textcolor{darkpastelred}{"Social Network"})} \\
\ourbench{} Environment: Error: Your service/namespace does not exist. \\
\reactname{}: \textit{Thought:} I should check the services deployed within the test-social-network namespace to ensure I use the correct service name. \\
\textit{Action:} I will list the services in the test-social-network namespace to confirm the correct name of the service. \\
\texttt{exec\_shell("kubectl get services -n test-social-network")}
\end{tcolorbox}


The \react{} agent had the highest token consumption for both model input and output.
This indicates that the \react{} agent's reasoning process engaged more heavily 
    when faced with minor formatting errors,
    which allowed it to achieve a relatively high detection accuracy of 76.92\%.
The \flash{} agent, sacrificing more cost 
    in the reasoning process,
    demonstrated the highest accuracy, 
    successfully detecting all of the faults.  

The non-agent-based anomaly detection method \mksmc{},
     which was much faster, with an average execution time of just 1 second. 
However, it only correctly identified 2 detection problems, 
    performing significantly worse than random guessing.

\insight{As the simplest task and the first step an AIOps agent should perform, 
    not all agent can successfully handle 
    the binary choice detection problems well in \ourbench{}.\label{finding:detection}}

\todo{Test the False Positive cases}








==> Makefile <==
# NAME := main
# TEXS := $(wildcard *.tex)
# TABLES := $(wildcard tables/*.tex)
# NUMBERS := $(wildcard numbers/*.tex)
# PLOTS := $(wildcard data/plots/*.eps)
# CODE := $(wildcard code/*.java)
# BIBS := $(wildcard *.bib)

# %.pdf: %.fig 
# 	fig2dev -L eps -f Roman $*.fig >$*.eps

# all: ${NAME}.pdf

# ${NAME}.pdf: ${TEXS} ${TABLES} ${NUMBERS} ${BIBS} ${CODE} ${PLOTS}
# 	-pdflatex $(NAME)
# 	-bibtex $(NAME)
# 	-pdflatex $(NAME)
# 	-pdflatex $(NAME)
# 	@echo '****************************************************************'
# 	# @dvips -t letter -o $(NAME).ps $(NAME).dvi
# 	# @ps2pdf -dPDFSETTINGS=/prepress $(NAME).ps $(NAME).pdf
# 	@echo '******** Did you spell-check the paper? ********'

# clean:
# 	ls $(NAME)* | grep -v ".tex" | grep -v ".bib" | xargs rm -f
# 	rm -f *.bak *~


# "Improved" Makefile for LaTeX documents
# INTPUFILE This defines the name of the file you want to latex
# the make file will automatically look for INPUT.tex as the latex file
INPUTFILE=main
# diffrev=8f0540d999d2178e216ec6f62415f5a3fa2d2726

default:
	latexmk -f -pdf ${INPUTFILE}
	@echo '****************************************************************'
	@echo '******** Did you spell-check the paper? ********'
	@echo '****************************************************************'

diff: diff.pdf
diff.pdf: diff.tex
.PHONY: diff.tex
diff.tex:
	latexdiff-vc --git --flatten \
		-r $(diffrev) \
		--append-textcmd="resizebox,multirow,caption,mrev" \
		--exclude-safecmd="mrev" \
		--disable-citation-markup \
		-c "PICTUREENV=(?:picture|DIFnomarkup|grammar|techreport|thebibliography|cite|tabular)[\w\d*@]*" \
		${INPUTFILE}.tex
	sed -e 's/\hspace{0pt}%DIFAUXCMD/\hskip0pt%DIFAUXCMD/g' ${INPUTFILE}-diff$(diffrev).tex > diff.tex
	rm ${INPUTFILE}-diff$(diffrev).tex

clean:
	latexmk -c ${INPUTFILE}
	rm -f ${INPUTFILE}.bbl

allclean:
	latexmk -C ${INPUTFILE}
	rm -f ${INPUTFILE}.bbl

monitor:
	latexmk -pdf -pvc ${INPUTFILE}

cleaner: allclean

view: ${INPUTFILE}.pdf
	open ${INPUTFILE}.pdf

${INPUTFILE}.pdf: default

count:
	texcount -brief *.tex



==> boxes.tex <==
\usepackage[most]{tcolorbox}
\usepackage{lipsum}
\usepackage{tocloft}
\usepackage{etoolbox}
\usepackage{mdframed}

\newcommand{\custombox}[2]{
  \begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=#1]
    #2
  \end{tcolorbox}
}


\newcommand{\agentbox}[2]{
  \begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,boxsep=0.5pt,title=Agent]
    \footnotesize{\textbf{Thought:} #1}\vspace{1.25pt}\\#2
  \end{tcolorbox}
}


\newcommand{\obsbox}[1]{
  \begin{tcolorbox}[colback=green!5!white,colframe=green!45!black,boxsep=0.5pt,title=Observation]
    \footnotesize{#1}
  \end{tcolorbox}
}

\newcommand{\orchbox}[1]{
  \begin{tcolorbox}[colback=gray!5!white,colframe=gray!75!black,boxsep=0.5pt,title=Orchestrator]
    \footnotesize{#1}
  \end{tcolorbox}
}


\newtcbox{\inlinebox}[1][]{enhanced, box align=base, nobeforeafter, colback=gray!10, colframe=gray!50, boxrule=0.5pt, arc=4pt, left=1pt, right=1pt, top=-1pt, bottom=-1pt, #1}

